CollabStory: Multi-LLM Collaborative Story Generation and Authorship Analysis

The rise of unifying frameworks that enable seamless interoperability of Large Language Models (LLMs) has made LLM-LLM collaboration for open-ended tasks a possibility. Despite this, there have not been efforts to explore such collaborative writing. We take the next step beyond human-LLM collaboration to explore this multi-LLM scenario by generating the first exclusively LLM-generated collaborative stories dataset called CollabStory. We focus on single-author to multi-author (up to 5 LLMs) scenarios, where multiple LLMs co-author stories. We generate over 32k stories using open-source instruction-tuned LLMs. Further, we take inspiration from the PAN tasks that have set the standard for human-human multi-author writing tasks and analysis. We extend their authorship-related tasks for multi-LLM settings and present baselines for LLM-LLM collaboration. We find that current baselines are not able to handle this emerging scenario. Thus, CollabStory is a resource that could help propel an understanding as well as the development of new techniques to discern the use of multiple LLMs. This is crucial to study in the context of writing tasks since LLM-LLM collaboration could potentially overwhelm ongoing challenges related to plagiarism detection, credit assignment, maintaining academic integrity in educational settings, and addressing copyright infringement concerns. We make our dataset and code available at https://github.com/saranya-venkatraman/CollabStory.

==> 7_misc.tex <==
% \begin{figure*}[t!]
%     \centering    \includegraphics[width=0.8\textwidth]{images/data_pipeline.pdf}
%     \caption{Rough outline, will make properly: Multi-LLM Story Generation Pipeline}
%     \label{fig:pipeline}
% \end{figure*}


\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc|cr}
\toprule
\# Number & \# Words per Author / & \# Author Order & \# Prompts per & \# Stories & Authors & \multicolumn{1}{c}{HuggingFace\footnotemark[3] distribution of LLMs used} \\
of Authors ($N$) & \# Total Words & Permutations & Author Order & & \\ \midrule
1 & 900 / 900 & 4 & 1800 & 7200 & Gemma & \texttt{google/gemma-1.1-7b-it}\footnotemark[4] \\
2 & 450 / 900 & 12 & 600 & 7200 & Llama & \texttt{meta-llama/Llama-2-13b-chat-hf}\footnotemark[5] \\
3 & 300 / 900 & 15 & 480 & 7200 & Mistral & \texttt{mistralai/Mistral-7B-Instruct-v0.2}\footnotemark[6] \\
4 & 225 / 900 & 15 & 480 & 7200 & Orca & \texttt{microsoft/Orca-2-13b}\footnotemark[7] \\
5 & 180 / 900 & 15 & 480 & 7200 & Olmo & \texttt{allenai/OLMo-7B-Instruct}\footnotemark[8] \\
\bottomrule
\end{tabular}%
}
\caption{Summary of Data Collection Statistics}
\label{tab:story_data_collection}
\end{table*}


% \paragraph{Catch As Catch Can} Style change detection is an advanced task where detectors must not only find all points where authorship changes within an article but also attribute each independent segment to the specific LLM author. {\dataset} is the first such resource with long-form stories written by multiple LLMs that can support the development and expansion of this authorship task and methods to help address incoming challenges brought by LLM interactions. As one example, this could affect academic integrity evaluations in classroom settings. As more and more LLMs become easier to combine, students might have different LLMs write various sections of an academic paper to evade current detectors.



